BKL bounces outside homogeneity: Gowdy symmetric spacetimes

We study the phenomenon of bounces, as predicted by Belinski, Khalatnikov and Lifshitz (BKL), as an instability mechanism within the setting of the Einstein vacuum equations in Gowdy symmetry. In particular, for a wide class of inhomogeneous initial data we prove that the dynamics near the $t = 0$ singularity are well-described by ODEs reminiscent of Kasner bounces. Unlike previous works regarding bounces, our spacetimes are not necessarily spatially homogeneous, and a crucial step is proving so-called asymptotically velocity term dominated (AVTD) behaviour, even in the presence of nonlinear BKL bounces and other phenomena such as spikes. (A similar phenomenon involving bounces and AVTD behaviour, though not spikes, can also be seen in our companion paper "BKL bounces outside homogeneity: Einstein-Maxwell-scalar field in surface symmetry", albeit in the context of the Einstein-Maxwell-scalar field model in surface symmetry.) One particular application is the study of (past) instability of certain polarized Gowdy spacetimes, including some Kasner spacetimes. Perturbations of such spacetimes are such that the singularity persists, but the intermediate dynamics -- between initial data and the singularity -- feature BKL bounces.

==> equations.tex <==
%auto-ignore

\section{The Einstein--Maxwell--scalar field system in surface symmetry} \label{sec:equations}

\subsection{Surface symmetric spacetimes} \label{sub:eqns_sss}

We consider \emph{surface symmetric} spacetimes, meaning spacetimes having one of spherical, plane, or hyperboloidal symmetry. Restricting to the \emph{trapped} region where the area-radius variable $r$ is timelike, such spacetime metrics $\mathbf{g}$ may be written in the following form, where $\Sigma = \mathbb{S}^2, \R^2, \mathbb{H}^2$ respectively.
\begin{equation} \label{eq:surface_sym}
    \mathbf{g} = - e^{2 \mu} dr^2 + e^{2 \lambda} d x^2 + r^2 d \sigma_{\Sigma}.
\end{equation}

Here $d \sigma_{\Sigma}$ denotes the standard metric on the surface $\Sigma$ with constant sectional curvature $\kappa \in \{1, 0 , -1\}$; %more precisely
\[
    d \sigma^2 = d \theta^2 + \sin_{\kappa}^2 \theta d \varphi^2 = 
    \begin{cases}
        d \theta^2 + \sin^2 \theta \, d \varphi^2 & \text{ if } \Sigma = \mathbb{S}^2, \\[-0.2em]
        d \theta^2 + d \varphi^2 & \text{ if } \Sigma = \R^2, \\[-0.2em]
        d \theta^2 + \sinh^2 \theta \, d \varphi^2 & \text{ if } \Sigma = \mathbb{H}^2.
    \end{cases}
\]
%We shall define $\kappa$ to be $+1$, $0$, or $-1$ depending on whether $\Sigma$ is $\mathbb{S}^2$, $\mathbb{R}^2$, or $\mathbb{H}^2$ respectively.

For a surface symmetric spacetime $(\mathcal{M}, \mathbf{g})$ which is a solution to the Einstein equations \eqref{eq:einstein}, if follows that the matter fields $\mathbf{\Phi}$ must also be surface symmetric in the following sense: the energy momentum tensor $\mathbf{T}[\mathbf{\Phi}]$ is described purely by (a) its projection onto the quotient manifold $\mathcal{Q} = \mathcal{M}/\!\!\sim$, and (b) its trace with respect to $d \sigma_{\Sigma}$. %-part of the metric. 
In other words, the remaining degrees of freedom of $\mathbf{T}_{\mu\nu}[\mathbf{\Phi}]$ are a two-tensor $T_{\mu\nu}$ on $\mathcal{Q}$ and a function $\mathbf{S}$ on $\mathcal{Q}$, given by
\[
    T_{\mu\nu} = \mathbf{T}_{\mu\nu} \text{ for } \mu, \nu \in \{ r, x \}, \quad \text{ and } \quad \mathbf{S} = \tr_{d \sigma_{\Sigma}} \mathbf{T} = \mathbf{T}_{\theta \theta} + \sin_{\kappa}^{-2} \theta \, \mathbf{T}_{\varphi \varphi}.
\]

Given this decomposition of the energy-momentum tensor $\mathbf{T}[\mathbf{\Phi}]$, we may express the Einstein equations \eqref{eq:einstein} with respect to the coordinates of \eqref{eq:surface_sym} as follows:
\begin{gather}
    \label{eq:lambda_evol_T}
    r \partial_r \lambda = r^2 T_{rr} - \frac{1}{2} \left( 1 + \kappa e^{2 \mu} \right), \\[0.8em]
    \label{eq:mu_evol_T}
    r \partial_r \mu = r^2 e^{2 (\mu - \lambda)} T_{xx} + \frac{1}{2} \left( 1 + \kappa e^{2 \mu} \right), \\[0.8em]
    \label{eq:mu_constraint_T}
    \partial_x \mu = r T_{xr}, \\[0.8em]
    \label{eq:mu_wave_T}
    \begin{split}
        (r \partial_r)^2 \mu - r^2 e^{2 (\mu- \lambda)} \partial_x^2 \mu = 
        & (r \partial_r \lambda) (r^2 \tr_{\mathcal{Q}} T + \kappa) e^{2\mu} + r \partial_r \left[ \left( r^2 \tr_{\mathcal{Q}} T + \kappa \right) e^{2 \mu} \right]  \\
        &\quad + r^2 e^{2 (\mu - \lambda)} \partial_x \mu \, \partial_x (\mu - \lambda) + r^2 e^{2 (\mu- \lambda)} \left[ T_{xx} - \frac{1}{2} \tr_{\mathcal{Q}} T e^{2 \lambda} - \frac{\mathbf{S}}{2} e^{2 \lambda} \right].
    \end{split}
\end{gather}
%
Furthermore, the wave equation $\square_{\mathbf{g}} \phi = 0$, written with respect to the coordinates of \eqref{eq:surface_sym}, is given by:
\begin{equation} \label{eq:phi_wave_T}
    (r \partial_r)^2 \phi - r^2 e^{2(\mu-\lambda)} \partial_x^2 \phi = e^{2 \mu} (r \partial_r \phi) \left( r^2 \tr_{\mathcal{Q}} T + \kappa \right) + r^2 e^{2(\mu-\lambda)} \partial_x \phi \, \partial_x (\mu - \lambda).
\end{equation}

\subsection{The EMSFSS system}

We now specialize the above to the Einstein--Maxwell--scalar field system, with Maxwell tensor $\mathbf{F}$ given by the following $2$-form, where $Q(r, x)$ is a function in $\mathcal{Q}$:
\begin{equation} \label{eq:maxwell_F}
    \mathbf{F} = \frac{2Q}{r^2} e^{\mu + \lambda} dr \wedge dx.
\end{equation}
For this system Maxwell's equations imply that $dQ = 0$, thus the Maxwell charge $Q$ is constant\footnote{For instance, one may check that $*\mathbf{F} = 2 Q d \theta \wedge \sin_{\kappa}\!\theta \, d \varphi$, while the second equation in \eqref{eq:maxwell} is equivalent to $d\! * \!\mathbf{F} - 0$}. In other words, the Maxwell field experiences no dynamics in this model, as we record in the following lemma:
\begin{lemma}
    Let $(\mathcal{M}, \mathbf{g}, \phi, \mathbf{F})$ be a surface symmetric solution to the Einstein--Maxwell--scalar field system \eqref{eq:einstein}--\eqref{eq:maxwell_em} with metric $\mathbf{g}$ given by \eqref{eq:surface_sym} and Maxwell tensor $\mathbf{F}$ given by \eqref{eq:maxwell_F}. Then $Q(r, x)$ is a constant.
\end{lemma}

We now specialize the remaining equations of Section~\ref{sub:eqns_sss} to the Einstein--Maxwell--scalar field model \eqref{eq:einstein}--\eqref{eq:maxwell_em} in the following proposition.

\begin{proposition}[Surface symmetric Einstein--Maxwell--scalar field system] \label{prop:emsfss_surface_sym} 
    Let $(\mathcal{M}, \mathbf{g}, \phi, \mathbf{F})$ be a surface symmetric solution to the Einstein--Maxwell--scalar field system \eqref{eq:einstein}--\eqref{eq:maxwell_em}, with metric $\mathbf{g}$ given by \eqref{eq:surface_sym} and Maxwell tensor $\mathbf{F}$ given by \eqref{eq:maxwell_F}. Then the dynamical quantities $(\lambda, \mu, \phi)$ satisfy the following equations for $(r, x) \in \mathcal{Q}$.
    \begin{gather}
        \label{eq:lambda_evol}
        r \partial_r \lambda = \frac{1}{2} \left( (r \partial_r \phi)^2 + r^2 e^{2(\mu - \lambda)} (\partial_x \phi)^2 - 1 - \kappa e^{2 \mu} + \frac{Q^2}{r^2} e^{2 \mu} \right), \\[0.8em]
        \label{eq:mu_evol}
        r \partial_r \mu = \frac{1}{2} \left( (r \partial_r \phi)^2 + r^2 e^{2(\mu - \lambda)} (\partial_x \phi)^2 + 1 + \kappa e^{2 \mu} - \frac{Q^2}{r^2} e^{2 \mu} \right), \\[0.8em]
        \label{eq:mu_constraint}
        \partial_x \mu = r \partial_r \phi \, \partial_x \phi, \\[0.8em]
        \label{eq:mu_wave}
        \begin{split}
            (r \partial_r)^2 \mu - r^2 e^{2 (\mu- \lambda)} \partial_x^2 \mu = 
            &e^{2 \mu} (r \partial_r \lambda) \left( - \frac{Q^2}{r^2} + \kappa \right) + r \partial_r \left[ e^{2 \mu} \left( - \frac{Q^2}{r^2} + \kappa \right) \right]  \\
            &\quad + r^2 e^{2 (\mu - \lambda)} \partial_x \mu \, \partial_x (\mu - \lambda) + 2 r^2 e^{2 (\mu- \lambda)} (\partial_x \phi)^2 - \frac{Q^2}{r^2} e^{2 \mu}, 
        \end{split} \\[0.8em]
        \label{eq:phi_wave}
        (r \partial_r)^2 \phi - r^2 e^{2(\mu-\lambda)} \partial_x^2 \phi = e^{2 \mu} (r \partial_r \phi) \left( - \frac{Q^2}{r^2} + \kappa \right) + r^2 e^{2(\mu-\lambda)} \partial_x \phi \, \partial_x (\mu - \lambda).
    \end{gather}
    Furthermore $\mu - \lambda$ obeys the transport equation 
    \begin{equation} \label{eq:mulambda_evol}
        r \partial_r (\mu - \lambda) = 1 + \left( - \frac{Q^2}{r^2} + \kappa \right) e^{2\mu}.
    \end{equation}
\end{proposition}


==> global.tex <==
%auto-ignore

\section{Global existence towards \texorpdfstring{$r = 0$}{t=0}}

The proof of Theorem~\ref{thm:global} will follow from a bootstrap argument. By local existence (Proposition~?), there exists some $r_b \in (0, r_0)$ such that a solution to the Einstein--Maxwell--scalar field system \eqref{eq:mu_evol}--\eqref{eq:phi_wave} exists in the interval $r \in [r_b, r_0]$, which moreover satisfies the bootstrap assumptions \eqref{eq:bootstrap_maxwell}--\eqref{eq:bootstrap_d2x}. 

Our goal will be to show that assuming this, we are able to improve upon the bootstrap assumptions, for instance by showing that \eqref{eq:bootstrap_maxwell}--\eqref{eq:bootstrap_d2x} hold with $C_*$ replaced by $C_*/2$. Therefore a standard continuity argument (using the continuation criterion?), one can allow $r_b$ to be any real number in the interval $(0, r_0)$, giving global existence towards $r = 0$.

For this purpose, let $(\phi, \mu, \lambda, Q)$ be a solution of the Einstein--Maxwell--scalar field system in our bootstrap region $r \in [r_b, r_0]$ with the initial data assumptions \eqref{eq:data_linfty}, \eqref{eq:data_linfty2} and \eqref{eq:data_energy_boundedness}. Then the results of Section~\ref{sec:l2} all apply, in particular Proposition~\ref{prop:energy_hierarchy}, Lemma~\ref{lem:low_order_linfty} and Corollary~\ref{cor:ode}. For convenience, let us record the result of Lemma~\ref{lem:low_order_linfty} again here: for $f \in \{ \phi, \mu, \lambda \}$ and $0 \leq k \leq 3$, there exists a family of constants $\updelta = \updelta( C_*, \upzeta, r_* )$ with $\updelta \downarrow 0$ as $r_* \downarrow 0$ so that
\begin{equation} \label{eq:low_order_linfty_copy}
    \| \partial_x^k f (r, \cdot) \|_{L^{\infty}} + \| r \partial_r \partial_x^k f (r, \cdot) \|_{L^{\infty}} \leq \updelta r^{-1/2}.
\end{equation}

The improvement of the bootstrap assumptions will be proceed in the following steps:

\medbreak \noindent
\underline{Step 1: ODE analysis on timelike curves:} 
\medbreak \noindent
The first step will be to use Corollary~\ref{cor:ode} and the results of Section~\ref{sec:ode} to provide $L^{\infty}$ bounds for the following $4$ key quantities:
\[
    r \partial_r \phi, \quad \frac{Q^2}{r^2} e^{2\mu}, \quad \partial_x \mu, \quad r \partial_r \partial_x \phi.
\]

To be more precise, let $\gamma: [r_b, r_0] \to \mathcal{Q}$ with $\gamma(r) = (r, x(r))$ be a $C^1$ \emph{past-directed timelike curve}, one example being a curve of constant $x$. In view of the metric \eqref{eq:surface_sym}, the fact that $\gamma(r)$ is timelike implies that one must have $|\frac{dx}{dr}| \leq e^{\mu - \lambda}$. For such a curve $\gamma(r)$, let us define
\begin{gather}
    \mathscr{P}(r) \coloneqq r \partial_r \phi ( \gamma(r)), \quad \mathscr{Q}(r) \coloneqq \frac{Q^2}{r^2} e^{2\mu} (\gamma(r)), 
    \label{eq:PQ_def} \\[0.6em]
    \mathscr{M}(r) \coloneqq \partial_x \mu ( \gamma(r)), \quad \mathscr{N}(r) \coloneqq r \partial_r \partial_x \phi ( \gamma (r)).
\end{gather}

Note that the initial data assumption \eqref{eq:data_linfty} implies that $\upeta^{-1} \leq \mathscr{P}(r_0) \leq \upeta$ and $\mathscr{Q}(r_0) \leq 1$. Furthermore, the assumption \eqref{eq:data_energy_boundedness}, together with Sobolev embedding on $\mathbb{S}^1$, implies there is a constant $C_{\mathbb{S}^1}$ independent of all parameters such that $|\mathscr{M}(r_0)|, |\mathscr{N}(r_0)| \leq C_{\mathbb{S}^1} \upzeta r_0^{-\upgamma}$. Furthermore, from \eqref{eq:P_ode_err}--\eqref{eq:Q_ode_err} of Corollary~\ref{cor:ode} with $a = a(r) = \frac{dx}{dr} \cdot (e^{\mu - \lambda})^{-1}$, one has
\begin{gather}
    \left| r \frac{d}{dr} \mathscr{P}(r) + \mathscr{P}(r) \mathscr{Q}(r) \right| \, (r, x) \leq \updelta r^{1/2}, \label{eq:P_ode_err_timelike} \\[0.6em]
    \left| r \frac{d}{dr} \mathscr{Q}(r) - \mathscr{Q}(r) \left( \mathscr{P}(r)^2 - 1 - \mathscr{Q}(r) \right) \right| \, (r, x) \leq \mathscr{Q}(r) \cdot \updelta r^{1/2}. \nonumber
\end{gather}

This is exactly what we need to apply the nonlinear ODE results of Lemma~\ref{lem:ode_bounce}. Therefore we have $(4 \upeta)^{-1} \leq \mathscr{P}(r) \leq 4 \upeta, \mathscr{Q}(r) \leq 16 \upeta^2$. But this is true for \underline{all} timelike curves in our bootstrap spacetime, including all constant $x$ curves, therefore for all $(r, x) \in [r_b, r_0] \times \mathbb{S}^1$, one has
\begin{equation} \label{eq:pq_improvement}
    (4 \upeta)^{-1} \leq r \partial_r \phi (r, x) \leq 4 \upeta, \qquad \frac{Q^2}{r^2} e^{2\mu} (r, x) \leq 16 \upeta^2.
\end{equation}

We move onto $\mathscr{M}(r)$ and $\mathscr{N}(r)$. Using now \eqref{eq:M_ode_err}--\eqref{eq:N_ode_err} from Corollary~\ref{cor:ode}, we also have
\begin{gather*}
    \left| r \frac{d}{dr} \mathscr{M}(r) + \mathscr{Q}(r) \mathscr{M}(r) - \mathscr{P}(r) \mathscr{N}(r) \right| \, (r, x) \leq \updelta r^{1/2}, \\[0.6em]
    \left| r \frac{d}{dr} \mathscr{N}(r) + 2 \mathscr{P}(r) \mathscr{Q}(r) \mathscr{M}(r) + \mathscr{Q}(r) \mathscr{N}(r) \right| \, (r, x) \leq \updelta r^{1/2}.
\end{gather*}
Together with the initial data assumption $|\mathscr{M}(r_0)|, |\mathscr{N}(r_0)| \leq C_{\mathbb{S}^1} \upzeta r_0^{-\upgamma}$, this is what we need to apply Lemma~\ref{lem:ode_variation} -- note the change from $\upzeta$ to $C_{\mathbb{S}^1} \upzeta$ is harmless. Therefore for some $D > 0$ depending on $\upeta$, $\upgamma$, $\upzeta$ but not on $C_*$, we have $|\mathscr{M} (r)| + |\mathscr{N} (r)| \leq D r^{-\upgamma}$. This is true for all timelike curves $\gamma(r)$, so for all $(r, x) \in [r_b, r_0] \times \mathbb{S}^1$,
\begin{equation} \label{eq:mn_improvement}
    | \partial_x \mu (r, x) | \leq D r^{-\upgamma}, \qquad |r \partial_r \partial_x \phi (r, x) | \leq D r^{- \upgamma}.
\end{equation}

\medbreak \noindent
\underline{Step 2: Improving the bootstrap assumption \eqref{eq:bootstrap_maxwell}} 
\medbreak \noindent
Note that by choosing $C_* \geq 32 \upeta^2$ and using \eqref{eq:pq_improvement}, we have already improved the first half of \eqref{eq:bootstrap_maxwell}. However, in order to improve the remaining parts of \eqref{eq:bootstrap_maxwell}, it will be necessary to upgrade the pointwise bound on $\frac{Q^2}{r^2} e^{2\mu}$ to an integrated bound on timelike curves.

More precisely, let $\gamma: [r_b, r_0] \to \R$ be a timelike curve as in Step 1. We rewrite the ODE-type estimate \eqref{eq:P_ode_err_timelike} in the following fashion, using crucially the lower bound for $r \partial_r \phi$ in \eqref{eq:pq_improvement}:
\[
    \left| r \frac{d}{dr} \log \mathscr{P}(r) + \mathscr{Q}(r) \right| \, (r, x) \leq 4 \upeta \updelta r^{1/2}.
\]
We now integrate this with respect to the differential $\frac{dr}{r}$. One finds:
\begin{equation*}
    \left| \int_r^{r_0} \mathscr{Q}(\tilde{r}) \frac{d\tilde{r}}{\tilde{r}} \right| \leq \left| \big [ \log \mathscr{P}(r) \big ]_r^{r_0} \right| + 4 \upeta \updelta \leq \log (16 \upeta^2) + 4 \upeta \updelta,
\end{equation*}
where the second inequality follows from the upper and lower bounds in \eqref{eq:pq_improvement}. We apply this estimate to the case where $\gamma(r) = (r, x)$ is a timelike curve of constant $x$; we have for $D_1 = \log(16\upeta^2) + 4 \upeta \updelta$ (which is crucially independent of $C_*$) the estimate
\begin{equation} \label{eq:Q_integral}
    \left| \int_r^{r_0} \frac{Q^2}{r^2} e^{2\mu} (\tilde{r}, x) \frac{d \tilde{r}}{\tilde{r}} \right| \leq D_1.
\end{equation} 

To apply this to improve bounds for $e^{2\mu}$ and $e^{2(\mu - \lambda)}$, we use the equations \eqref{eq:lambda_evol} and \eqref{eq:mu_evol} to derive that
\begin{gather}
    r \partial_r (r^{-1} e^{2\mu}) = \left( (r \partial_r \phi)^2 + r^2 e^{2(\mu - \lambda)} (\partial_x \phi)^2 + \kappa e^{2\mu} - \frac{Q^2}{r^2} e^{2\mu} \right) r^{-1} e^{2\mu} \geq \left( - e^{2\mu} - \frac{Q^2}{r^2} e^{2\mu} \right) r^{-1}e^{2\mu}, \label{eq:reu_eq} \\[0.6em]
    r \partial_r (r^{-1} e^{2(\mu - \lambda)}) = \left( 1 + 2 \kappa e^{2\mu} - \frac{2 Q^2}{r^2} e^{2\mu} \right) r^{-1} e^{2(\mu - \lambda)} \geq 2 \left( - e^{2\mu} - \frac{Q^2}{r^2} e^{2\mu} \right) r e^{2(\mu - \lambda)}. \label{eq:reum_eq}
\end{gather}

Using the bootstrap assumption \eqref{eq:bootstrap_maxwell} and that $r_* \geq r_0$ may be chosen small, let us choose $r_*$ so that alongside \eqref{eq:Q_integral}, we have that $\int^{r_0}_r e^{2\mu} (\tilde{r}, x) \frac{d \tilde{r}}{\tilde{r}} \leq 1$. Then integrating \eqref{eq:reu_eq} and \eqref{eq:reum_eq} along constant $x$-curves, as well as applying the initial data assumption \eqref{eq:data_linfty2},
\begin{gather*}
    r^{-1} e^{2\mu} (r, x) \leq e^{D_1 + 1} r_0^{-1} e^{2\mu}(r_0, x) \leq e^{D_1 + 1} \upzeta, \\[0.6em]
    r^{-1} e^{2(\mu - \lambda)} (r, x) \leq e^{2(D_1 + 1)} r_0^{-1} e^{2(\mu - \lambda)} (r_0, x) \leq e^{2(D_1 + 1)} \upzeta.
\end{gather*}
Thus for $C_*$ chosen larger than $2 e^{2(D_1 + 1)} \upzeta$, we may improve the latter part of \eqref{eq:bootstrap_maxwell}.

\medbreak \noindent
\underline{Step 3: Improving the bootstrap assumption \eqref{eq:bootstrap_rdr}} 
\medbreak \noindent

We have already improved the bootstrap assumption for $|r \partial_r \phi|$ in \eqref{eq:bootstrap_rdr} because of \eqref{eq:pq_improvement}, so long as we choose $C_* \geq 8 \upeta$. To improve $|r \partial_r \lambda|$ and $|r \partial_r \mu|$, we simply use \eqref{eq:lambda_evol} and \eqref{eq:mu_evol}. Using Lemma~\ref{lem:low_order_linfty} to estimate the term involving $\partial_x \phi$, and using both \eqref{eq:pq_improvement} and $e^{2\mu} \leq e^{D_1 + 1} \upzeta r$ and $e^{2(\mu - \lambda)} \leq e^{2(D_1 + 1)} \upzeta r$ from Step 2, %we get:
\begin{align*}
    | r \partial_r \lambda | 
    &\leq \frac{1}{2} \left( (r \partial_r \phi)^2 + r^2 e^{2(\mu - \lambda)} (\partial_x \phi)^2 + 1 + e^{2\mu} + \frac{Q^2}{r^2} e^{2\mu} \right) \\[0.6em]
    &\leq \frac{1}{2} \left( 16 \upeta^2 + e^{2 (D_1 + 1)} \upzeta \updelta^2 r^{3 - 2 \upgamma} + 1 + e^{D_1 + 1} \upzeta r  + 16 \upeta^2 \right).
\end{align*}
Using also $r \leq r_0 \leq 1$, the right hand side is bounded independent of $C_*$, and thus by choosing $C_* \geq 2 \cdot \mbox{RHS}$, we have improved the bootstrap assumption for $|r \partial_r \lambda|$. The improvement for $|r \partial_r \mu|$ follows from an identical calculation.

\medbreak \noindent
\underline{Step 4: Improving the bootstrap assumptions \eqref{eq:bootstrap_dx} and \eqref{eq:bootstrap_d2x}} 
\medbreak \noindent

We complete the proof by improving the remaining bootstrap assumptions \eqref{eq:bootstrap_dx} and \eqref{eq:bootstrap_d2x}. We start with the \eqref{eq:bootstrap_d2x}, noting that the bootstrap assumption for $|r \partial_r \partial_x \phi|$ is already improved due to \eqref{eq:mn_improvement}, so long as $C_* \geq 2D$.

To improve the bootstrap assumptions for $|r \partial_r \partial_x \lambda|$ and $|r \partial_r \partial_x \mu|$, we simply differentiate \eqref{eq:lambda_evol} and \eqref{eq:mu_evol} with respect to $x$, then combine several previously found estimates. Differentiating \eqref{eq:lambda_evol} yields
\[
    r \partial_r \partial_x \lambda = (r \partial_r \phi) (r \partial_r \partial_x \phi) + r^2 e^{2(\mu - \lambda)} \partial_x (\mu - \lambda) (\partial_x \phi)^2 + r^2 e^{2(\mu - \lambda)} \partial_x \phi \, \partial_x^2 \phi - \kappa e^{2\mu} \partial_x \mu + \frac{Q^2}{r^2} e^{2\mu} \partial_x \mu.
\]
Therefore using all of \eqref{eq:pq_improvement}, \eqref{eq:mn_improvement}, Lemma~\ref{lem:low_order_linfty} and the estimates for $e^{2\mu}$ and $e^{2(\mu - \lambda)}$ in Step 2, one yields
\[
    |r \partial_r \partial_x \lambda| \leq (4 \upeta D + e^{2(D_1 + 1)} \upzeta D^3 r^{3 - 2 \upgamma} + e^{2(D_1+ 1)} \upzeta D^2 r^{3 - \upgamma} + e^{D_1 + 1} \upzeta D r + 16\upeta^2 D ) r^{- \upgamma}.
\]
One can carry out an identical calculation for $|r \partial_r \partial_x \mu|$. Therefore for some $D_2$ independent of $C_*$, one has
\begin{equation} \label{eq:b4_improvement}
    |r \partial_r \partial_x \phi|, |r \partial_r \partial_x \lambda|, |r \partial_r \partial_x \mu| \leq D_2 r^{- \upgamma}.
\end{equation}

Finally, to improve \eqref{eq:bootstrap_dx}, we integrate \eqref{eq:b4_improvement} from $r = r_0$, and use the initial data assumption \eqref{eq:data_energy_boundedness} -- together with Sobolev embedding -- to get $|\partial_x \phi (r_0)| + |\partial_x \mu (r_0)| + |\partial_x \lambda (r_0)| \leq C_{\mathbb{S}^1} \upzeta r_0^{-\upgamma}$. Thereby integrating \eqref{eq:b4_improvement} yields:
\begin{equation} \label{eq:b3_improvement}
    |\partial_x \phi|, |r \partial_r \partial_x \lambda|, |r \partial_r \partial_x \mu| \leq (D_2 \upgamma^{-1} + C_{\mathbb{S}^1} \upzeta) r^{- \upgamma}.
\end{equation}

Thus upon choosing $C_* \geq 2 ( D_2 \upgamma^{-1} + C_{\mathbb{S}^1} \upzeta)$, \eqref{eq:b4_improvement} and \eqref{eq:b3_improvement} improve the remaining bootstrap assumptions \eqref{eq:bootstrap_d2x} and \eqref{eq:bootstrap_dx}. By the standard bootstrap argument, this concludes the proof of Theorem~\ref{thm:global}. (The two estimates \eqref{eq:global_linfty} and \eqref{eq:global_energy} follow from \eqref{eq:pq_improvement} and Proposition~\ref{prop:energy_hierarchy} respectively.)



